C3G: Learning Compact 3D Representations with 2K Gaussians

Reconstructing and understanding 3D scenes from unposed sparse views in a feed-forward manner remains as a challenging task in 3D computer vision. Recent approaches use per-pixel 3D Gaussian Splatting for reconstruction, followed by a 2D-to-3D feature lifting stage for scene understanding. However, they generate excessive redundant Gaussians, causing high memory overhead and sub-optimal multi-view feature aggregation, leading to degraded novel view synthesis and scene understanding performance. We propose C3G, a novel feed-forward framework that estimates compact 3D Gaussians only at essential spatial locations, minimizing redundancy while enabling effective feature lifting. We introduce learnable tokens that aggregate multi-view features through self-attention to guide Gaussian generation, ensuring each Gaussian integrates relevant visual features across views. We then exploit the learned attention patterns for Gaussian decoding to efficiently lift features. Extensive experiments on pose-free novel view synthesis, 3D open-vocabulary segmentation, and view-invariant feature aggregation demonstrate our approach's effectiveness. Results show that a compact yet geometrically meaningful representation is sufficient for high-quality scene reconstruction and understanding, achieving superior memory efficiency and feature fidelity compared to existing methods.

==> figure/tex/feature_field.tex <==
    \begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/assets/3dfeaturefield.pdf}
    \caption{\textbf{Qualitative results of feature lifting (place holder.}} 
    \label{fig:teaser}
\end{figure*}


==> figure/tex/intro_comparison.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth, height=0.3\linewidth]{example-image-duck}
    \caption{\textbf{Comparison of conventional 3DGS methods.} (a) Per-scene optimization (b) Feed-forward pixel-aligned 3DGS (c) Ours} 
    \label{fig:teaser}
\end{figure*}


==> figure/tex/number_of_gaussian.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/assets/gaussian_number.pdf}
    \caption{\textbf{Number of Gaussians ablation.}} 
    \label{fig:num_gaussian}
\end{figure}


==> figure/tex/qual_recon.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth, height=0.5\linewidth]{example-image-duck}
    \caption{\textbf{Qualitative results of novel view synthesis.}} 
    \label{fig:teaser}
\end{figure*}


==> figure/tex/vis_attention_map.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/assets/only_attn_vis.pdf}
    \caption{\textbf{Visualization of attention map (placeholder).}} 
    \label{fig:attn_vis}
\end{figure}


==> supple_sec/supple_table/different_number_of_view.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Comparison of novel view synthesis with multi-view input images.} Our method generates fewer Gaussians while achieving competitive or superior quality. $^\dagger$: applied test-time optimization of Gaussians. }
\label{suptab:multiview_nvs}
\vspace{-5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
% \multicolumn{15}{c}{ACID} \\
% \midrule
\multirow{2}{*}{Methods} & \multicolumn{4}{c|}{12 view} & \multicolumn{4}{c|}{24 view} & \multicolumn{4}{c}{36 view} \\
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & \#G$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & \#G$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & \#G$\downarrow$ \\
\midrule
AnySplat~\cite{jiang2025anysplat} & 23.057& 0.807& 0.215& 1,500K& 24.105& 0.838& 0.198 & 2,636K& 24.196& 0.842& 0.192& 3,309K\\ 
AnySplat$^\dagger$~\cite{jiang2025anysplat} & 26.726& 0.881& 0.189& 1,500K& 27.471& 0.898& 0.180 & 2,636K& 27.412& 0.899& 0.181& 3,309K\\ 
VGGT+NoPo~\cite{wang2025vggt, ye2024no} & 21.262& 0.667& 0.200& 602K& 21.244& 0.664& 0.200& 1,204K& 21.190& 0.663& 0.200& 1,806K\\ 
VGGT+NoPo$^\dagger$~\cite{wang2025vggt, ye2024no} & 28.540& \textbf{0.898}& \textbf{0.131}& 602K& 28.463& 0.902& \textbf{0.135}& 1,204K& 28.100& 0.898& 0.145& 1,806K\\ 


Ours & 23.612& 0.740& 0.203& \textbf{2K}& 23.797& 0.747& 0.198 & \textbf{2K}& 23.812& 0.747& 0.199& \textbf{2K}\\
Ours$^\dagger$ & \textbf{28.552}& 0.890& 0.155& 28K& \textbf{29.987}& \textbf{0.916}& 0.136& 27K & \textbf{30.250}& \textbf{0.921}& \textbf{0.133}& 26K\\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table*}

==> supple_sec/supple_table/n_view_feature_lifting.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{multi-view extension of feature lifting.} }
\label{suptabmulti-view feature}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{l|ccc|ccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{\shortstack{\shortstack{feed\\forward}}} & \multirow{2}{*}{\shortstack{Number of\\inputs}} & \multirow{2}{*}{\shortstack{Number of\\forward}} & \multicolumn{5}{c}{Lseg~\cite{li2022language}} \\
& & & & mIoU$\uparrow$ & Acc.$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
Feature-3DGS~\cite{zhou2024feature} & \ding{55} & N & - & 0.379& 0.644& 19.83& 0.684& 0.357\\
CF$^3$~\cite{lee2025cf3}& \ding{55} & N & - & 0.376& 0.657& 20.04& 0.691& 0.359\\
\midrule
Ours & \ding{51} & 2 & N & 0.513& 0.783& 23.89& 0.770& 0.285\\
Ours & \ding{51} & 24 & 1 & & & & & \\
\bottomrule
\end{tabular}}
\end{table*}

==> supple_sec/supple_table/probe3d_fit3d.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Correspondence estimation on ScanNet.} We evaluate PCK@10px across two images captured from different angle. Our feature aggregation significantly improves correspondence accuracy with the DINOv2-Base backbones.}
\label{suptab:correspondence}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|c}
\toprule
Methods & $\theta_{0}^{15}$ & $\theta_{15}^{30}$ & $\theta_{30}^{60}$ & $\theta_{60}^{180}$ & Avg. \\
\midrule
DINOv2-Base~\cite{oquab2023dinov2} & 36.9& 29.2& 19.3& 9.9& 23.8\\
FiT3D~\cite{yue2024improving} & 40.9& 32.1& 22.0& 13.9& 27.2\\
% DINOv2-base~\cite{oquab2023dinov2} + AnyUp~\cite{wimmer2025anyup}& 36.2 & 28.6 & 19.7 & 10.9 & 23.9\\
DINOv2-Base~\cite{oquab2023dinov2} + Ours & \textbf{92.9} & \textbf{88.4} & \textbf{70.5} & \textbf{22.2} &  \textbf{68.5}\\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table}

==> supple_sec/supple_table/upsampling.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Correspondence estimation on ScanNet with upsampled feature.} We evaluate PCK@10px across two images captured from different angle. Our feature aggregation significantly improves correspondence accuracy with the DINOv2-Base, DINOv2-Large and DINOv3-Large backbones.}
\label{suptab:upsampler}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|c}
\toprule
Methods & $\theta_{0}^{15}$ & $\theta_{15}^{30}$ & $\theta_{30}^{60}$ & $\theta_{60}^{180}$ & Avg. \\
\midrule
DINOv2-Base~\cite{oquab2023dinov2} & 36.9& 29.2& 19.3& 9.9& 23.8\\
DINOv2-Base~\cite{oquab2023dinov2} + AnyUp~\cite{wimmer2025anyup}& 36.2 & 28.6 & 19.7 & 10.9 & 23.9\\
DINOv2-Base~\cite{oquab2023dinov2} + Ours & \textbf{92.9} & \textbf{88.4} & \textbf{70.5} & \textbf{22.2} &  \textbf{68.5}\\
\midrule
DINOv2-Large~\cite{oquab2023dinov2} & 36.6& 24.0& 19.0& 12.7& 23.1\\
DINOv2-Large~\cite{oquab2023dinov2} + AnyUp~\cite{wimmer2025anyup}& 39.4& 25.5& 19.1& 14.0& 24.5\\
DINOv2-Large~\cite{oquab2023dinov2} + Ours & \textbf{94.2}& \textbf{89.0}& \textbf{70.5}& \textbf{21.0}& \textbf{68.7}\\
\midrule
DINOv3-Large~\cite{simeoni2025dinov3} &  54.9& 44.3& 32.1& 19.3& 37.7\\
DINOv3-Large~\cite{simeoni2025dinov3} + AnyUp~\cite{wimmer2025anyup}& 48.4& 34.8& 27.1& 16.8& 31.8\\
DINOv3-Large~\cite{simeoni2025dinov3} + Ours & \textbf{94.2}& \textbf{89.1}& \textbf{70.8}& \textbf{20.9}& \textbf{68.8}\\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table}

==> table/coarse_reconstruction.tex <==

\begin{table}[t]
\centering
\caption{\textbf{Comparison of novel view synthesis with limited number of Gaussians.} }
\label{tab:coarse_reconstruction}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{Methods}  & \multicolumn{4}{c}{Average} \\
&  PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & \#G \\
\midrule
Sampling & 21.340& 0.665& 0.272& 2K \\
Voxelize & 19.957& 0.609& 0.403& 4K \\
Ours & 22.387& 0.713& 0.259& 2K \\
\bottomrule
\end{tabular}}
\end{table}

==> table/feature_lifting_replica_known_view.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc|ccccc|ccccc|cc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Feature} & \multirow{2}{*}{\shortstack{Feed\\Forward}} & \multirow{2}{*}{\shortstack{Additional\\Input}} & \multicolumn{5}{c|}{LSeg~\cite{li2022language}}& \multicolumn{5}{c|}{MaskCLIP~\cite{zhou2022extract}} & & \\
& & & & mIoU$\uparrow$ & Acc$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & mIoU$\uparrow$ & Acc$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & \#G & Memories \\
\midrule
LSeg / MaskCLIP$^*$~\cite{li2022language, radford2021learning} & \ding{51} & \ding{55} & - & 0.647& 0.896& -& -& -& 0.414& 0.674& -& -& -& -& -\\
Feature-3DGS~\cite{zhou2024feature} & \ding{51} & \ding{55} & $\mathcal{I},\mathcal{P}$ & & & & & & & & & & & & \\ 
CF$^3$~\cite{} & \ding{51} & \ding{55} & $\mathcal{I},\mathcal{P}$ & & & & & & & & & & & & \\
\midrule
% PixelSplat~\cite{} & \ding{55} & \ding{51} & $\mathcal{I},\mathcal{P}$ & & & & & & & & & & & & \\
NoPoSplat~\cite{ye2024no} & \ding{55} & \ding{51} & $\mathcal{I}$ & -& -& 24.36& 0.809& 0.141& -& -& 24.36& 0.809& 0.141& & \\
% NoPoSplat$^\dagger$~\cite{ye2024no} & \ding{55} & \ding{51} & & -& -& & & & & & & & & 131K & \\
\midrule
LSM~\cite{fan2024large} & \ding{51} & \ding{51} & $\mathcal{I}$ & 0.600& 0.823& 19.271& 0.760& 0.230& & & & & & & \\
Ours & \ding{51} & \ding{51} & - & 0.649& 0.894& 25.347& 0.815& 0.177& 0.421& 0.695& 25.07& 0.811& 0.185& 2K& \\
\bottomrule
\end{tabular}}
\caption{\textbf{Comparison of feature novel view synthesis on Replica dataset.} $\dagger$: Reproduced results without using intrinsic information. $*$: Results after directly forward the target view images. $\mathcal{I}$: intrinsic, $\mathcal{P}$: extrinsic.}
\label{tab:benchmark_results}
\end{table*}

==> table/feature_lifting_scannet_known_view.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc|ccccc|ccccc|cc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Feature} & \multirow{2}{*}{\shortstack{Feed\\Forward}} & \multirow{2}{*}{\shortstack{Additional\\Input}} & \multicolumn{5}{c|}{LSeg~\cite{li2022language}}& \multicolumn{5}{c|}{MaskCLIP~\cite{zhou2022extract}} & & \\
& & & & mIoU$\uparrow$ & Acc$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & mIoU$\uparrow$ & Acc$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & \#G & Memories \\
\midrule
LSeg / MaskCLIP$^*$~\cite{li2022language, radford2021learning} & \ding{51} & \ding{55} & - & 0.521& 0.820& -& -& -& 0.344& 0.665& -& -& -& -& - \\
Feature-3DGS~\cite{zhou2024feature} & \ding{51} & \ding{55} & $\mathcal{I},\mathcal{P}$ & & & & & & & & & & & & \\ 
CF$^3$~\cite{} & \ding{51} & \ding{55} & $\mathcal{I},\mathcal{P}$ & & & & & & & & & & & & \\
\midrule
NoPoSplat~\cite{ye2024no} & \ding{55} & \ding{51} & $\mathcal{I}$ & -& -& 25.20& 0.812& 0.217& -& -& 25.20& 0.812& 0.217& & \\
\midrule
LSM~\cite{fan2024large} & \ding{51} & \ding{51} & $\mathcal{I}$ & 0.511& 0.798& 25.44& 0.811& 0.214& 0.251& 0.516& 25.012& 0.824& 0.230&          & \\
Ours & \ding{51} & \ding{51} & - & 0.542& 0.803& 23.92& 0.766& 0.278& 0.361& 0.668& 23.386& 0.759& 0.284& & \\
\bottomrule
\end{tabular}}
\caption{\textbf{Comparison of feature novel view synthesis on scannet dataset.} $\dagger$: Reproduced results without using intrinsic information. $*$: Results after directly forward the target view images. $\mathcal{I}$: intrinsic, $\mathcal{P}$: extrinsic.}
\label{tab:benchmark_results}
\end{table*}

==> table/multi_view_reconstruction.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Comparison of novel view synthesis with 24 input images.} Our method generates fewer Gaussians while achieving competitive or superior quality. $^\dagger$: applied test-time optimization of Gaussians. }
\label{tab:benchmark_results}
\vspace{-5pt}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{4}{c}{Average} \\
&  \#G$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
AnySplat~\cite{jiang2025anysplat} &  2636K & 24.105& 0.838& 0.198\\
AnySplat$^\dagger$~\cite{jiang2025anysplat}&  2636K & 27.471& 0.898& 0.180\\
\midrule
Ours & 2K& 23.797& 0.747& 0.198 \\
Ours$^\dagger$& 27K & 29.987& 0.916& 0.136\\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table}

==> table/novel_view_synthesis.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Comparison of novel view synthesis on RealEstiate10K.} Our method maintains competitive results while using far fewer Gaussians. $^\dagger$: Reproduced with VGGT backbone.}
\label{tab:nvs_baseline}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|cccccc}
\toprule
\multirow{2}{*}{\shortstack{\textit{Pose-}\\\textit{free}}} & \multirow{2}{*}{Methods} & \multicolumn{6}{c}{Average} \\
& & \#G $\downarrow$ & Memories$\downarrow$ & FPS$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
\multirow{2}{*}{\ding{55}} & PixelSplat~\cite{charatan2024pixelsplat} & 131K & 33.6MB &388.03 &  23.848  & 0.806 & 0.185 \\
& MVSplat~\cite{chen2024mvsplat}& 131K & 33.6MB &392.6 & 23.977 & 0.811 & 0.176 \\
\midrule
\multirow{8}{*}{\ding{51}} & CoPoNeRF~\cite{hong2024unifying}  & -& -&0.4 & 18.938 & 0.619 & 0.388\\
& Splatt3R~\cite{smart2024splatt3r} &131K & 33.6MB &393.1& 15.318 & 0.490 & 0.436 \\
& PF3plat~\cite{hong2024pf3plat}&131K & 33.6MB &397.1 & 21.042 & 0.739 & 0.233 \\
& SPFSplat~\cite{huang2025no}&131K & 33.6MB &397.3 & 25.845& 0.852& 0.152\\
& NoPoSplat~\cite{ye2024no} & 131K & 33.6MB &369.8& 25.033& 0.838& 0.160\\
& VGGT+NoPo$^\dagger$~\cite{wang2025vggt, ye2024no}& 100K & 25.6MB &419.8 & 23.015& 0.762& 0.187\\
& Ours & 2K & 0.1MB & 451.7& 22.387& 0.713& 0.259\\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table}

